Scalable and Probabilistic Leaderless BFT Consensus through Metastability

This paper introduces a family of leaderless Byzantine fault tolerance protocols, built around a metastable mechanism via network subsampling. These protocols provide a strong probabilistic safety guarantee in the presence of Byzantine adversaries while their concurrent and leaderless nature enables them to achieve high throughput and scalability. Unlike blockchains that rely on proof-of-work, they are quiescent and green. Unlike traditional consensus protocols where one or more nodes typically process linear bits in the number of total nodes per decision, no node processes more than logarithmic bits. It does not require accurate knowledge of all participants and exposes new possible tradeoffs and improvements in safety and liveness for building consensus protocols. The paper describes the Snow protocol family, analyzes its guarantees, and describes how it can be used to construct the core of an internet-scale electronic payment system called Avalanche, which is evaluated in a large scale deployment. Experiments demonstrate that the system can achieve high throughput (3400 tps), provide low confirmation latency (1.35 sec), and scale well compared to existing systems that deliver similar functionality. For our implementation and setup, the bottleneck of the system is in transaction verification.

==> Makefile <==

LATEX=TZ='UTC' pdflatex

BIBTEX=bibtex
BIBFILE=paper
PAPER=paper
TEXFILES = $(wildcard *.tex) $(wildcard sections/*.tex) $(wildcard figures/*.tex) $(wildcard figures/*.pdf)

SUBDIRS =
#figs

all: subdirs $(PAPER).pdf

subdirs:
	@for dir in $(SUBDIRS); do $(MAKE) -C $$dir; done;

$(PAPER).pdf: $(TEXFILES) $(BIBFILE).bib usenix2019_v3.sty
	$(LATEX) $(PAPER)
	$(BIBTEX) $(BIBFILE)
	$(LATEX) $(PAPER)
	$(LATEX) $(PAPER)

cleantex:
	rm -f *.aux *.log *~ *.out .DS_Store *.dvi $(PAPER).ps $(PAPER).pdf \
		*.lot *.lof *.toc *.blg *.bbl *.ent *.bak *.glo *.gls *.ist

clean: cleantex
	for dir in $(SUBDIRS); do $(MAKE) -C $$dir clean; done;\



==> obsolete/extra.tex <==
\section{Core Snowball Network Overlay Protocol}
In the discussion of the Snowball protocol we initially assumed a logically fully-connected network of nodes. 
Later, we relaxed that assumption and showed how the network view set intersection between correct nodes can have disjoint subsets and still maintain safety and liveness. 

In this section, we introduce the concrete details of the Snowball network overlay protocol, \textit{SNO}, whose function is to allow the network nodes to maintain a highly-up-to-date view of all active nodes in the system, i.e. allow for churn.
Beyond that, SNO also provides other useful features, including partial detection and prevention of Byzantine behavior, as well as network participation incentivization, which becomes important in the instantiation of the Snowball-based payment system \textit{SnoCoin}. 

\subsection{Background}
SNO makes usage of the core ideas of the Fireflies\cite{johansen2006fireflies} network overlay protocol, but modifies certain operational details. 
The Fireflies protocol forms a ring-based pseudorandom mesh from a network of $\mathcal{N}$ nodes, such that each node has a total of $\mathcal{O}(\log{|\mathcal{N}|})$ neighbors, and such that even if up to half of the neighbors are Byzantine, each correct node will maintain a highly up-to-date view of the entire set of active nodes. 

As before, we still assume for simplicity a logically fully connected network of nodes $\mathcal{N}$.
Each correct node, however, will only need to maintain $\mathcal{O}(\log{|\mathcal{N}|})$ network links.
Let each node $u \in \mathcal{N}$ have some unique identifier, represented by $u$.id, and let \texttt{H} be a secure cryptographic hash function that is pre-image and collision resistant. 
We generate a set of $\log |\mathcal{N}|$ ``rings'', where each ring -- indexed by $i$ such that $1 \leq i \leq 2*|\mathcal{B}| + 1$ -- is an ordering of the nodes based on the output of \texttt{H}($u$.id $||$ $i$), i.e. 
\[
    u.\text{\texttt{pos}}[i] = \text{\texttt{H}}(u.\text{\texttt{id}} || i); \forall u \in \mathcal{N}, 1 \leq i \leq 2|\mathcal{B}| + 1
\]
Nodes have two neighbors (two closest ordered nodes) on each ring, and all nodes can publicly verify the neighbors of other nodes. The first and last nodes wrap around and are always neighbors with each other on every ring. 

The Fireflies overlay guarantees, with high probability, that there exists a path between any two nodes and that this path is pseudorandom. 
Nodes periodically ping other nodes using the pseudorandom mesh generated by the rings structure, and based on the responses can accuse other nodes of failure. 
If a node is accused falsely, then the node may provide evidence of liveness. 
Using this mechanism, each node will maintain a reasonably up-to-date view of all the active nodes in the network and consequently weed out any failed nodes.  
We point the reader to the Fireflies paper for formal proofs.

\subsection{Snowball Network Overlay}
We use the network overlay construction in the Fireflies protocol, but modify it to act as the carrier of messages in the network, rather than just ping nodes periodically.
Every node $u$ chooses the set of $k$ random solicited nodes exactly as before (i.e. from the set of all nodes $\mathcal{N}$). 
This means that the semantics and interface of the Snowball core protocol remain exactly unmodified. 
However, rather than communicate with the solicited nodes directly, the solicitor queries along one of the random paths induced by the random communication mesh. 

For example, suppose that node $u$ chooses a random sample $\mathcal{R} \subset \mathcal{N}_u$ of size $k$ of nodes to solicit, and suppose that the shortest path to node $v \in \mathcal{R}$ is through node $g \in \mathcal{N}_u$. 
$u$ then transmits the message first to $g$, which will queue and forward it to $v$. 

On top of merely forwarding messages, $u$ and $g$ will keep track of the response by $v$. Untimely responses by $v$ will raise accusations by both $u$ and $g$. Enough accusations will result in all correct nodes removing $v$ from their respective network view. 

{\color{blue} Kevin: Expand the subsection here with a more formal protocol description. It should basically be the same as the Fireflies protocol. }

\section{Instantiation}
We now instantiate a payment system with Snowball, called SnoCoin. Before discussing the technical details, we discuss challenges and introduce the solutions adopted in this paper. 

\subsection{Sybils}
\label{subsection:sybil}
Any open and unprotected network can trivially become a victim to a Sybil attack~\cite{douceur2002sybil}, wherein an adversary can cheaply generate a large number of identities and take down the network. 
In Bitcoin, Sybils are deterred through the protocol-level usage of cryptographic puzzles, whose mathematical properties ensure that participation in decision making in the network is costly. 
Since Snowball does not make usage of proofs-of-work, alternative measures must be adopted. 
There are several techniques that may be used. 
Fundamentally, these techniques rely on trading one resource for authorization to participate in the system, but there are big practical differences between the actual resource chosen.
\begin{itemize}
\item IPv4 Scarcity: Many existing peer-to-peer systems, including Bittorrent and Bitcoin, employ Sybil deterrence at their network layer based on the scarcity of IPv4 addresses. 
Specifically, they observe that the IPv4 address space is densely allocated, and that it is difficult for an adversary to amass large numbers of addresses across the Internet.
Bitcoin's main mechanism against eclipse attacks coupled with low-difficulty chain construction is to ensure that a node peers with a diverse set of peers from multiple IP prefixes. 
One possibility, inspired by this mechanism, is to limit the number of participants per prefix. 
Coupled with an IANA-provided map of IP prefix allocations, this may help limit the number of Sybil nodes that an attacker, who has access to a limited number of machines and networks, can bring into the system.
\item Proof-of-Bond: A bond, denominated in the Snowball currency itself to eliminate any dependency on external resources, may be used to raise the costs to launch an attack. 
In this scheme, entry into the system requires the nodes to put up a bond for the duration of their stay in the system. 
This ensures that an attacker has to tie up significant amounts of cash to mount an attack.
Note that this is quite different from traditional proof-of-stake protocols in that it does not suffer from nothing-at-stake, the participants cannot retroactively rewrite history using stale keys, and the bond is not at risk of being usurped by the system.
\item Proof-of-Uniqueness: It is possible to require participants in Snowball to provide a proof-of-uniqueness provided by a secure hardware mechanism. 
One possibility is for every node to run a small, predetermined program in an SGX-like enclave and obtain a certificate that they executed the code on a genuine secure processor. 
This program can then issue just a single random number, derived from the on-chip secret.
\item External Credentials: In domains where the participants are issued a unique credential by an external entity, this credential can be used to authorize the node's entry into the system.
For instance, in settings where participants are issued unique certificates, they may join the network with a join transaction that takes the credential as an input. 
The network can then ensure that any given credential is used by at most one node.

\end{itemize}

SnoCoin adopts a combination of the first two measures to deter participants. We envision SNO to provide a platform for global remittance with the least amount of friction to participation. We envision potentially hundreds of thousands to millions of Internet-connected low-powered devices (such as mobile devices), transacting at peak capacity. Plainly speaking, a combination of the two provides the least amount of resistance for individual honest clients, but provides a reasonable deterrence to an adversary willing to spawn off millions of clusters around the world. 

% \subsection{View and Identity Management}
% {\color{blue}{Kevin: This section is of crucial importance, and needs to be precisely described.}}

% As discussed previously, an inconsistent view amongst correct nodes increases the ability of Byzantine nodes to affect both liveness and safety of the system. 
% Several mechanisms can be used to ensure a highly consistent view, but in SNO we make usage of a two-phase mechanism. 
% In the first phase, we use the proof-of-bond for providing membership into the network. 
% All nodes can authenticate the membership of all other nodes by simply verifying that the bond has been posted. 
% In the second phase, we make usage of Fireflies\cite{johansen2006fireflies}, an intrusion-tolerant network overlay protocol, which provides correct nodes a reasonably fresh view of the set of active nodes in the network, whilst tolerating a Byzantine presence with up to half of all active nodes.
% Constructing such a network overlay provides several benefits. 
% First, it allows correct nodes to efficiently prune out inactive nodes, increasing efficiency of polling in the Snowball protocol. 
% Second, it provides a clean means of rewarding good behavior. 
% Correct nodes that participate and stay active in the network may request rewards in the system in the form of coin minting in SNO. 

\subsection{Failure Detection}

\subsection{Network Congestion Control}
In our analysis, we assumed a Byzantine adversary with powers that, in reality, are extremely difficult to achieve. A large body of work on network congestion control is highly applicable to any instantiation of Snowball. Several relevant techniques are:
\paragraph{Randomized backoff} Whenever a correct node is queried, the node can randomly choose a wait time before responding to the querying node. Although this simple technique makes no distinction between nodes, it is still extremely efficient in reducing the ability of Byzantine nodes to mount attacks. 
\paragraph{Targetted backoff} Additionally, a correct node may keep track of the frequency of requests for each neighbor, and respond to requests accordingly. 

% \subsection{Network View}
% \label{subsection:networkview}
% As in any active open network, it is hard to guarantee that the network view is consistent amongst all correct nodes. 
% In Snowball, we make usage of intrusion tolerant network overlays in order to 

\section{Extra Text}

The advantage of linking the transactions together rather than running
repetitive voting process for each isolated one is two-fold. On the one hand,
the proper policy will create a positive feedback that once a transaction is
supported by most nodes out of its conflict sets, it will become increasingly
likely to be supported in the future.

On the other hand, it makes the system scalable regarding the total number of
transactions, because for each node in the network, every transaction only need
to be voted once.  When the node asks for votes for a newly discovered
transaction, the voting result transitively contributes to all the ancestor
transactions on the DAG\@.  Without the DAG, conflict sets are free-floating with
their transactions, so one has to keep polling for the votes for transactions
in all conflict sets, even the confidence values of oldest ones are rocksolid to
reach a consensus. The reason we have to repeat voting in absence of a DAG is
for a practical system, especially an electronic cash system, any node
should be able to recover from incorrect temporary state seamlessly
to achieve an eventual consistency. This means the consensus protocol is
theoretically always running, but the probabilistic safety guarantee gets
improved over time, so the decision threshold is just an observation from the
current process of consensus and guides the business decisions (e.g.\ whether
to render the service or deliver the goods).  Bitcoin uses the longest chain
rule to represent the current state (decisions) of the transactions, and when a
block is appended to the chain, it enhances the belief on all the preceding
blocks.

Gossip-based protocols are usually designed to work in settings where the nodes
are benign. However, in our system, where Byzantine behavior could present,
some extra care is taken to improve the security given the attackers could push
around incorrect information and disrupt decision making.

The core protocol is mainly pull-based. That is, the only ``pushed''
information is the transaction data, which do not affect the decision process.
Transaction data are neutral, and transactions themselves do not play a role in
making decisions until they are polled. A node only runs the protocol based on
the local information gathered from voting summary sampled at random and will
never need to trust others. The only external information other than
transaction data is the polling result from the sampled nodes. But because the
sampling is controlled by the poller, the attackers could not affect the voting
result if they are not asked, nor could they force the set of nodes to be
polled. There is no exchange of voting result or confidence value between the
nodes. The belief of the chosen transactions are autonomously built by active
sampling and polling, on behalf of the node itself.

2.


The extensive past work on Byzantine consensus can be divided into two families: permissioned and permissionless consensus protocols. 

\paragraph{Permissioned BFT Consensus}
The seminal protocol PBFT~\cite{castro1999practical} protocol was the first Byzantine consensus protocol to guarantee low transaction latency and safety for a network of $3|\mathcal{B}|+1$ nodes.  
PBFT entails quadratic $\mathcal{O}(|\mathcal{N}|^2)$ message complexity and its guarantees break down non-gracefully with bound violation. 
Abd-El-Malek et al.~\cite{abd2005fault} and Cowling et al.~\cite{cowling2006hq} use a quorum-based approach to optimize for contention-free cases of operation to achieve consensus in only a single round of communication. 
However, although these protocols improve on performance, they degrade very poorly under contention. 
Zyzzyva~\cite{kotla2007zyzzyva} couples BFT with speculative execution to improve the failure-free operation case. 
Guerraoui et al.~\cite{guerraoui2010next} introduce a protocol with optimized performance under several -- rather than just one -- cases of execution. 
In contrast, Clement et al.~\cite{clement2009making} sacrificed some performance to tolerate worst-case degradation, providing a more uniform execution profile. 
This work, in particular, sacrificed failure-free optimizations to provide consistent throughput even at high number of failures. 

Other past work in permissioned BFT systems typically requires at least $2|\mathcal{B}|+1$ replicas tolerance. 
However, work in 2012 by Kapitza et al.~\cite{kapitza2012cheapbft} showed how to leverage trusted hardware components to construct a protocol that uses $|\mathcal{B}|+1$ replicas. 

On the other end of the spectrum, other work attempts to introduce new protocols under redefinitions and relaxations of the BFT model. 
Rodrigues et al.~\cite{rodrigues2007large} modify PBFT to allow for arbitrary choice of number of replicas and failure threshold, providing a probabilistic guarantee of liveness for some failure ratio but protecting safety with high probability. 
Such relaxation of the BFT protocol is a core design principle of Snowball, where we postulate that for a payment system such as SnoCoin, safety is far more important than liveness. 
In another form of relaxation, the work of Singh et al.~\cite{singh2009zeno} introduced a BFT state machine replication protocol that trades consistency for high availability. 
More specifically, this paper guarantees eventual consistency rather than linearizability, meaning that participants can be inconsistent but eventually agree once the network stabilizes. 
By providing an even weaker consistency guarantee, namely fork-join-causal consistency, in 2011 Mahajan et al.\cite{mahajan2011depot} described a protocol that guarantees safety under $|\mathcal{B}|+1$ replicas. 

\paragraph{Permissionless BFT Consensus}
Bitcoin~\cite{nakamoto2008bitcoin} was the first protocol to show the possibility of consensus under no predefined set of identities. The core insight is the usage of proof-of-work (PoW) to replace voting by identities with voting by computational power. While techniques based on proof-of-work~\cite{dwork1992pricing,aspnes2005exposing}, and even cryptocurrencies with minting based on proof-of-work~\cite{vishnumurthy2003karma,rivest1997payword}, had been explored before, Bitcoin was the first to incorporate PoW into its consensus process.

Bitcoin, however, has at least two major weaknesses: performance and scale. 
Bitcoin incurs high confirmation latency at around 10 minutes, is hard-capped at 7 transactions/sec maximum throughput, and exhibits significant short-term variance in both of these metrics due to its mining protocol -- it is not uncommon for transactions to take much more than an hour to confirm. 
These fundamental protocol limits pose problems for the protocol's scale~\cite{croman2016scaling}. 
Further, nodes can take up to a few days to start up, as validating the blockchain involves vetting every single transaction since the deployment of the system. 
The MimbleWimble~\cite{mimblewimble} proposal promises to save on disk storage by pruning spent transactions through homomorphic cryptography. 

In the last two years, a flurry of protocols that tackle scale and efficiency of Bitcoin have been proposed. 
Bitcoin-NG~\cite{eyal2016bitcoin} refactors the creation of blocks such that block dissemination is no longer a bottleneck.
In a similar fashion, both Pass et al.~\cite{pass2016hybrid} and ByzCoin~\cite{kokoris2016enhancing} make use of the underlying PoW mechanism to choose quorums to process transactions in each epoch, using PBFT.
Luu et al.~\cite{luusharding2016} similarly use PoW to create logarithmic-sized shards upon which protocols like PBFT can be run.
All of these systems still rely crucially on proof of work, and thus do not tackle a crucial inefficiency.

Proof of stake (PoS) protocols, which employ variants of PBFT among a cohort of nodes whose desired behavior is incentivized through a financial bond, have been suggested as a way to replace computationally wasteful proofs of work. 
While there have been many PoS proposals~\cite{peercoin,NXT,steem,casper,bentovpoa}, few of them have any associated proof of correctness.
Algorand~\cite{micali2017algorand}, Snow White~\cite{bentovsnow} and Ouroboros~\cite{kiayias2016provably} are some of the earliest provably secure proof-of-stake (PoS) protocols. Of these, Snow White provides the strongest guarantees, as it provides both liveness and safety for a system of at most half adversarial nodes. 

{\color{blue}Kevin: further discussions need to go here about related works. There is some stuff in the related works section that maybe doesn't even really belong all that much, and definitely some stuff that's kind of missing, especially in the latest wave of work.}


------------------------------------------------------------------------------------------------

\section{Future Work}
\begin{itemize}
    \item \textbf{Network Model}: we conjecture this protocol family also works
        under a partially synchronous network assumption. This is because the
        sampling and querying process makes the system self-synchronized,
        and our current randomized global scheduler model is weaker
        than the round-based model used by strongly synchronized protocols.
        A new model or model transformation is expected.
    \item \textbf{Minting}: in order to build a decentralized cryptocurrency,
        we need a minting mechanism that incentivizes correct behavior of nodes.
    \item \textbf{Membership}: to build a permissionless system, a complete
        staking and unstaking mechanism needs to be implemented, which may fusion into
        the existing Avalanche protocol to benefit from its safety guarantees.
    \item \textbf{Joining}: since Avalanche has relatively high throughput,
        it may take very long time for a new node to catch up the entire history of DAG using
        the existing mechanism.
\end{itemize}



==> obsolete/oldtheta1.tex <==
% -------------
% DO NOT DELETE.
% DO NOT DELETE.
% DO NOT DELETE.
% -------------
Every correct node is chosen by the scheduler at most a fixed number of times, $\delta$, after which the value of every correct node is collected and counted.
Note another (and final) condition: if a node is selected and that node has seen $\phi$ consecutive majorities for the same value, it no longer updates its value, regardless of the output of the polling. 

\subsubsection{Safety of \Theta_1}
The expression for the hypergeometric experiment is reasonably complex, and it becomes hard to reason about the different ways that each of the variables inside the expression affects the outcomes. In particular, it is not clear how network size affects the experiment. This is of interest because if the effect of network size has little bearing on the outcomes of the experiment, it has important consequences for the scalability of the $\Theta_1$ protocol. To see how network size affects the system, we can fortunately make usage of the 

\subsubsection{Adversarial Optimality}
We will first try to determine the optimal strategy that the Byzantine
adversary can play.  Once we have this strategy, we will analyze how
effective this strategy is.
Recall that we do not care about violating liveness for conflicting
transactions, so the adversary's objective is to violate
safety, that is, it wants some correct node to decide red while another
correct node decides blue.  

As a thought experiment, consider that most correct nodes lean red
while only one correct node leans blue.  Given our sampling protocol,
it is clear that if there are not too many Byzantine nodes, the red-leaning
nodes will continue to lean red, while the blue-leaning node will
start increasing its confidence in red and eventually become red-leaning
as well.  It thus stand to reason that a primary objective of the adversary
is to have half of the correct nodes lean red, while the other half lean
blue, and to keep it this way.

However, the adversary faces a conflict.  Consider that the adversary
has only limited time ($\phi$ rounds) to accomplish its goal of
violating safety.  When half the nodes are leaning blue, and half
the nodes are leaning red, their confidence in either blue or red
will not grow rapidly, and they likely will not decide in the limited
amount of time.  Also, if some node $u$ is close to deciding blue
and a small majority of nodes are leaning blue, then if $u$ polls
a Byzantine node it is not clear whether the Byzantine node should
return red or blue.  If the Byzantine node returns blue, it may
cause $u$ to decide blue but still give the adversary a chance to
get other nodes to decide red.  If the Byzantine node returns red,
it may help restore the balance between red- and blue-leaning nodes.

This conflict for the adversary illustrates exactly the strength of
the Snowball protocol.  While it is relatively easy for the adversary
to prevent deciding on conflicting transactions, it is difficult for
the adversary to cause two correct nodes to decide different transactions.

\begin{comment}
If this is the situation, then if a correct
node samples other nodes, it will, by expectation, receive the same number of
red and blue votes from the correct nodes that it samples.

The Byzantine strategy then is straightforward:
if there are as many red-leaning nodes as blue-leaning nodes and
a red-leaning node samples from a Byzantine node, the Byzantine node
returns red, and vice versa.
If the node has equal confidence in red or blue, it does not matter
which color the Byzantine node returns and can, say, flip a coin.
If, however, the system is not in balance, and
there are more red than blue nodes, then a Byzantine node will always
``push back'' by returning blue (and vice versa).
We will later demonstrate that this strategy is optimal.

Next, we need to show that although optimal, the strategy cannot
cause a violation of safety with high probability.
We will show that whp no 
correct node ever decides (if there are conflicting values), and in particular
no two correct nodes ever disagree.
If the Byzantine strategy is non-optimal, correct nodes may decide, but
they will decide the same value whp.
\end{comment}

\begin{comment}
We define \emph{skew} as the maximum among the distances between the
confidence vectors (interpreted as points in a Euclidean space)
of correct node pairs.  For example, if there are three correct nodes
with confidence vectors $\langle 0, 3 \rangle$, $\langle 1, 3 \rangle$,
and $\langle 4, 0 \rangle$, then the skew is~5 (the distance between
the first and last confidence vector endpoints).
The optimal strategy for the Byzantine nodes is to maximize skew.

% TODO: Expand in sentences the notation written about maximal policy below. 
We want to characterize \textit{drift} in the differences of values between any two correct nodes. Specifically, letting the absolute difference between the values of any correct node correspond to some confidence differential, represented by $\max_{\Delta}(u) = u[0]-u[1]$ if $|u[0]| > u[1]$ and $\max_{\Delta}(u) = u[1]-u[0]$ if $u[1] > |u[0]|$, we desire to precisely quantify bounds on the maximum drifts between any two correct nodes, and for all possible execution instances $\mathcal{I}_i$. In other words, what is the execution path $\mathcal{I}_{opt}$ such that
\[
    \mathcal{I}_{opt}(\mathcal{C}^{t_0}) = \max_{\forall i}\{\mathcal{I}_i(\mathcal{C}^{t_0})\}
\]
where
\[
    \mathcal{I}_{i}(\mathcal{C}^{t_0}) = \max_{\forall u, v \in \mathcal{C}^{t_\phi}}\{\max_{\Delta}(u)-\max_{\Delta}(v)\}
\]
To exactly characterize the probability of a safety failure of the optimal execution path, we would need to calculate the probability distribution over all possible permutations of Byzantine answers, which is a function of the choices of execution of the correct nodes as well as the distribution of the choices of the neighbors.
In other words, over all possible execution paths (i.e. there are $c$ nodes to choose at each time step, for a total of $\phi^{c}$ ways of choosing over $\mathcal{C}$ nodes) and over all possible choices of the $k$-sampled neighbors (for a total of ${n \choose k}$ such choices, per node, per execution round), we would need to keep track of all of the possible tuples of the Byzantine value updates. 
Generating such a stochastic model would, plainly speaking, be infeasible. 
\end{comment}

\paragraph{Optimality Condition}
We can simplify the analysis greatly if we fix the Byzantine strategy to some optimal policy, $\mathcal{A}_{\pi}$. 
Let $s$ be a three-tuple where the first entry is a color configuration of the set of nodes in $\mathcal{C}$ (i.e. the set $\lbrace(u_1[\mathtt{R}], u_1[\mathtt{B}]), (u_2[\mathtt{R}], u_2[\mathtt{B}]), \dots, (u_c[\mathtt{R}], u_c[\mathtt{B}])\rbrace$, where $u[\mathtt{R}], u[\mathtt{B}] \in [0, \phi]$), the second entry is the chosen node at some round $u \in \mathcal{C}$ in round $t_i$, and the third entry is the round itself $t_i$. Let $\mathtt{S}$ be the set of all such tuples $s$. The elements of $\mathtt{S}$ are the necessary pieces of information needed for the Byzantine strategy. 
For each state $s \in \mathtt{S}$, the set of allowable actions for the Byzantine nodes is either $\mathtt{R}$ or $\mathtt{B}$. Let $P(s' | s, {\mathtt{R}})$ be the probability of transitioning from state $s$ to $s'$ given that the Byzantine strategy responds with $\mathtt{R}$, and conversely for $\mathtt{B}$. Let $\mathtt{Z}(s)$ be the reward for entering state $s$. Let the policy $\mathcal{A}_{opt}(s)$ be the optimal policy which returns the color chosen by the Byzantine node at state $s$, given round $i$. 
The utility $\mathcal{U}$ of $s$ (and the optimal policy) are then defined as
\begin{equation}
\begin{split}
\mathcal{U}(\mathcal{A}_{opt}, s) =\ \mathtt{Z}(s)\ +& \sum_{s' \in S} P(s' | s, \mathcal{A}_{opt}(s))\\
\times &\ \mathcal{U}(\mathcal{A}_{opt}, s')
\end{split}
\end{equation}
where 
\begin{equation}
\begin{split}
    \mathcal{A}_{opt}(s) &= \argmax_{a \in \lbrace \mathtt{R}, \mathtt{B} \rbrace} \left \lbrace \sum_{s' \in S}P(s'|s, a)\mathcal{U}(\mathcal{A}_{opt}, s') \right \rbrace
\end{split}
\end{equation}
These are the equations that follow from Bellman's optimality principle. Note that we do not include a discount factor. Further, we assign a reward of 1 to the states where there exists two nodes $u, v$ such that $\gamma_u \geq \gamma$ and $\gamma_v \leq 1/\gamma$. 

Since the state space is computationally infeasible, we solve for the optimal policy inductively, rather than iteratively. 
Let $count(\mathcal{C}^{t_i}, \mathtt{R})$ be defined as: 
\begin{equation}
\begin{split}
    count(\mathcal{C}^{t_i}, \mathtt{R}) = \sum_{u \in \mathcal{C}^{t_i}} \mathbbm{1}(u, \mathtt{R})
\end{split}
\end{equation}
where $\mathbbm{1}$ is the indicator function defined as:
\begin{equation}
\begin{cases}
    \mathbbm{1}(u, \mathtt{R}) = 1\ \text{\textbf{if}}\ u[\mathtt{R}] > u[\mathtt{B}]\\
    \mathbbm{1}(u, \mathtt{R}) = 0\ \text{\textbf{if}}\ u[\mathtt{R}] < u[\mathtt{B}]\\
    \mathbbm{1}(u, \mathtt{R}) = \{1, 0\}\ \text{\textbf{if}}\ u[\mathtt{R}] == u[\mathtt{B}]\ \text{\textbf{and} $u$ lastly}\\
    \text{preferred $\{\mathtt{R}, \mathtt{B}\}$}
\end{cases}
\end{equation}
and conversely for $count(t_i, \mathtt{B})$. 

Let $\mathcal{C}_{\mathtt{R}}$ be the set of correct nodes that the Byzantine nodes color as red at the cold start phase, and $\mathcal{C}_\mathtt{R}$ the converse. It is easy to see that a coloring of equal split between red and blue in the cold-start phase is the optimal configuration for a single iteration of the $\Theta_1$ protocol. It is not clear, however, how this configuration must evolve (if at all) as time progresses. 

Let $\mathcal{A}_\pi$ be the chosen Byzantine strategy described formally in Figure \ref{figure:mathcal_a_pi}. 
\begin{figure}[h!]
\label{figure:mathcal_a_pi}
\fbox{
    \parbox{0.95\linewidth}{
        \begin{center}
            \textbf{The $\mathcal{A}_\pi$ policy}
        \end{center}
        Let the Byzantine nodes set $\mathcal{C}_\mathtt{R}$ to be exactly half of the correct nodes in the network, and $\mathcal{C}_\mathtt{B}$ the other half at the cold-start phase. We initialize a local memory $\mathds{M}$, which stores various information about the history of execution up to step $t_i$. Let $\{\mathcal{C}', u, t_i\} \leftarrow s$, where $\mathcal{C}^{t_i} = \mathcal{C}'$ (note that there are multiple valid versions of $\mathcal{C}^{t_i}$, nevertheless in this case we refer to the specific set $\mathcal{C}$ extracted from state $s$). 
        \begin{itemize}
            \item If $count(\mathcal{C}^{t_i}, \mathtt{R}) = c/2$:
            \subitem In this case, the set of correct nodes is equally split. If $u \in \mathcal{C}_\mathtt{R}$, then all Byzantine nodes are colored red. Conversely for blue. Add $s$ to $\mathds{M}$, and return. 
            \item If $count(\mathcal{C}^{t_i}, \mathtt{R}) < c/2$:
            \subitem In this state, the set of correct nodes has shifted to a majority blue. This implies that at some time step $t_j < t_i$, a node $v \in \mathcal{C}_\mathtt{R}$ gained at least 1 extra confidence for blue than for red. Locate this node $v$ by searching the history stored in memory $\mathds{M}$. Move $v$ to the corresponding color assignment, i.e. set $\mathcal{C}_\mathtt{R} = \mathcal{C}_\mathtt{R}\backslash v$ and $\mathcal{C}_\mathtt{B} = \mathcal{C}_\mathtt{B} \cup v$. Search in $\mathcal{C}^{t_i}$ for all nodes $v'$, s.t. $\mathbbm{1}(v', \mathtt{B}) = 1$, and find the $v'$ with the minimum skew between blue and red, i.e. $\min \{v'[\mathtt{B}] - v'[\mathtt{B}]\} \forall v'$. Move the target $v'$ to the opposite color assignment, i.e. set $\mathcal{C}_\mathtt{B} = \mathcal{C}_\mathtt{B}\backslash v'$ and $\mathcal{C}_\mathtt{R} = \mathcal{C}_\mathtt{R} \cup v'$. Finally, if $u \in \mathcal{C}_\mathtt{R}$, then all Byzantine nodes are colored red. Conversely for blue. Add $s$ to $\mathds{M}$, and return. 
        \end{itemize}
    }
}
\end{figure}

\begin{comment}
    \begin{algorithm}
    \begin{algorithmic}[1]
    \Procedure{$\mathcal{A}_\pi$}{$s$}
    \State $\{\mathcal{C}', u, t_i\} \leftarrow s$
    \If{$\mathbbm{1}(u, \mathtt{R})$} \Comment{$u$ prefers $\mathtt{R}$}
    \If{$u \in \mathcal{C}_\mathtt{R}$}
    \State
    \EndIf
    \EndIf
    \State $\mathcal{A}(u, \mathcal{C})$ \Comment{Deterministic Byzantine strategy}
    \State $s \xleftarrow{\$^k} \mathcal{N}$\textbackslash $u$
    \If{count($s, \mathtt{R}$) $\geq$ $\alpha k$}
    \State $u[\mathtt{R}]~ += 1$
    \EndIf
    \If{count($s, \mathtt{B}$) $\geq$ $\alpha k$}
    \State $u[\mathtt{B}]~ += 1$
    \EndIf
    \State update($\mathcal{C}$, $u$)
    \EndProcedure
    \end{algorithmic}
    \end{algorithm}
\end{comment}

\begin{theorem}
The Byzantine strategy $\mathcal{A}_\pi$ is optimal, i.e. $\mathcal{A}_\pi = \mathcal{A}_{opt}$.
\end{theorem}
\begin{proof}
We inductively prove the claim. 
The base case is when the nodes are equally split in half, i.e. $count(\mathcal{C}^{t_i}, \mathtt{R}) = c/2$. Let $\mathcal{H}_{\mathcal{N}, c/2 + b + j}^k/\mathcal{H}_{\mathcal{N}, c/2 - j}^k$ represent the expected ratio growth of $\gamma_u$, where $u \in \mathcal{C}^\mathtt{R}$. 
Naturally, this ratio grows as $j$ grows (i.e. as the number of red-preferring correct nodes increases). 
However, the converse is also true, meaning that as $j$ increases, the $\gamma_v$ ratio for $v \in \mathcal{C}_\mathtt{B}$ decreases at the same rate. 
In particular, this rate is poly-exponential, meaning that even small changes to $j$ incur large benefits (and conversely penalties) on the confidence ratios. 
Therefore, the optimal split between correct nodes that maximizes the probability of $\gamma_u > \gamma_v$ and $\gamma_v > 1/\gamma$ where $u$ prefers red and $v$ prefers blue is when $j = 0$. 
In the usual case, the Byzantine nodes initially label the correct nodes equally between red and blue, and respond with red whenever a red-labelled correct node samples, and blue whenever a blue-labelled correct node samples. 
However, in the case when an initially red-labelled node (i.e. $u \in \mathcal{C}_\mathtt{R}$) suddenly switches confidence to blue, the Byzantine node must update it's strategy. 
The Byzantine nodes have three options: either keep responding red to the newly switched node, update responses to blue, or choose a new node and update its colors. 
Since every selection by the scheduler is uniformly at random, the expected number of times a node will be selected starting from time $t_i$ is equal amongst all correct nodes and is exactly $\phi - i / c - 1$. 
Therefore, in expectation, there is no difference between $u$ and a node $v$ which prefers the same color and which has no bigger skew than $u$. 
Sticking to the prior color labelling is clearly suboptimal since the growth of $\gamma_*$ of the new majority color will be larger than the minority color. Therefore, the optimal strategy is to simply pick the node of same color as the newly flipped node that has the \textit{minimum} skew (i.e. confidence) in its color. 
\end{proof}

Under no adversarial presence, the progress made by correct nodes is equal, in expectation, amongst all honest nodes. More formally, let $\mathcal{B} = \emptyset$. Then, $\forall u^{t_i}, v^{t_i} \in \mathcal{C}^{t_i}$, $i \geq 0$, 
\[
    \mathbb{E}[u^{t_i}[\mathtt{R}]] = \mathbb{E}[v^{t_i}[\mathtt{R}]]
\]
\[
    \mathbb{E}[u^{t_i}[\mathtt{B}]] = \mathbb{E}[v^{t_i}[\mathtt{B}]]
\]
At any time-step, the probability of each correct node being selected and subsequently adding either a red ball or blue ball is a function of the underlying number of red and blue preferences, but otherwise equal and uniform among all nodes. In Lemma \ref{lemma:expected_absorption}, we computed the expected number of steps to reach the state where all nodes prefer red. Upon reaching this state, every new added color will be the same, and growth of the opposing color will be zero. 

If Byzantine nodes are introduced, the expectation changes as a function of the underlying Byzantine strategy. Let $p_q^l(\mathtt{R}, \mathcal{S}, k, \alpha)$ be the probability of achieving at least $l$ consecutive successes for the color red over a sequence of $q$ trials given that $\mathcal{S}$ nodes in the network $\mathcal{N}$ prefer red. We let $\epsilon < 1$ be a security parameter, and after fixing $q$, we solve for the minimal value of $l$ such that 
\[
    p_q^l(\mathtt{R}, c, k, \alpha) \leq \epsilon
\]
In other words, we compute the minimal number of consecutive support for red until, with probability no more than $\epsilon$, at least $c$ nodes in the network also prefer red. 

It is easy to see that the probability is equal between the opposing colors as well as maximal when $\mathcal{S} = c/2 + b$. However, this probability is clearly much smaller than $\mathcal{O}(\epsilon^2)$. Suppose that the Byzantine nodes deviate from the optimal strategy in order to render the probability of committing at least one color to some value greater than $\epsilon$. In that case, the Byzantine nodes must allow the correct nodes to swing away from an equal network split. 

At this point in the deviation of the strategy, the ``snowball'' effect of $\Theta_1$ becomes apparent and highly compounded. Let $c/2 + \delta$ represent the expansion of the number of correct nodes towards red, and $c/2 - \delta$ the contraction of the number of correct nodes towards blue. Using the result from a prior lemma, the ratio of the speed of absorption will now be $g(c/2 + \delta)$. 

\begin{comment}
========= END PHASE 1

Fortunately, we can make usage of a useful observation: the probability of two independent successes for \texttt{opposing} values for any pair of hypergeometric experiments is maximum only when the frequency of the values in the network is exactly equal. 
To prove this, we simply need to solve for $i$ in the following expression: 

\begin{equation}
\max \{P(\mathcal{H}_{n, i}^k \geq \alpha k)*P(\mathcal{H}_{\mathcal{N}, n-i}^k \geq \alpha k)\}, 0 \geq i \geq n
\end{equation}

This probability is increases exponentially quickly as $i \rightarrow n/2$, with a maximum at $n/2$, and an exponential dropoff from $i = n/2$ to $n$. 
This observation is tremendously helpful because it allows us to fix the Byzantine adversary to a single optimal strategy: force the correct nodes into two equally split partitions, and -- throughout all $\delta$ executions -- put all the Byzantine nodes towards answering the corresponding value to each partition. 
Any other split, including non-fixed dynamic Byzantine strategies, would incur lower probability of success. 

Following on our observation, we can now fix the Byzantine strategy to the following: at time $t_0$, the Byzantine nodes choose two equal partitions of correct nodes, and for each subsequent time step, every Byzantine node will answer $1$ whenever the first partition queries and $2$ whenever the second partition queries. 

The probability that we receive $\phi$ or more successes over $\delta$ trials is a complicated expression, whose exact value requires a recursive expression. We leave the reader to Feller\cite{feller1} (Vol 1. Sec. XIII.7) for more information. Let $\mathcal{U}_{\delta}(\mathcal{H}_{\mathcal{N}, C^{t_i}}^k)$ be the random variable that outputs the number of consecutive successes of the hypergeometric experiment over $\delta$ trials. 
Then, the probability that a specific correct node receives $\phi$ or more consecutive successes is then: 

\begin{equation}
P_{consecutive} = \frac{1}{|\mathcal{C}|}P(\mathcal{U}_{\delta}(\mathcal{H}_{\mathcal{N}, C^{t_i}}^k) \geq \phi)
\end{equation}

The probabilities are symmetric across all correct nodes. Therefore, the probability of safety failure ($P_{sf}$) over all possible $|\mathcal{C}/2|^2$ pairs of correct nodes is then: 

\begin{equation}
    P_{sf} = |\mathcal{C}/2|^2 * P_{consecutive}^2
\end{equation}

The probabilities of safety failure are shown in Figure \ref{fig:safety_failure}.

\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{./figures/safety_failure.pdf}
\caption{Probability of safety failure, $\phi = 20$, $\delta = 100$, $|\mathcal{N}| = 500$, and $k = 10$, for various size of Byzantine nodes and $\alpha k$.}
\label{fig:safety_failure}
\end{figure}

% \subsubsection{Liveness of \Theta_1}
% A key metric related to liveness is convergence latency, the amount of time between the introduction of a value proposal to the time every correct node agress on the same value.
% Described in terms of network configurations, this convergence latency calculates the expected number of rounds from any bivalent network configuration until reaching a state where all correct nodes vote for the same value. 
% We first show that convergence latency for a Byzantine-free network is logarithmic in the size of the network. Later, we calculate bounds on the maximum adversarial size that still guarantees expected logarithmic convergence. 
% Let the system be initialized to state $\psi = \{|\mathcal{C}_1^{t_0}|, |\mathcal{C}_2^{t_0}|\}$. 
% We perform a Markovian analysis on the probabilities of transitioning to any of all the possible states arising from $\psi$. 
% The state space $\mathbb{S}$ of all possible configurations arising from $\psi$ is all possible bivalent network splits between values $1$ and $2$, such that $|\mathcal{C}_1^{t_0}| + |\mathcal{C}_2^{t_0}| = |\mathcal{N}|$. 
% As an example, suppose the total number of correct nodes is 100. Then, all possible states of the system are $\{0, 100\}, \{1, 99\}, \dots, \{100, 0\}$.
% We can now construct the transition probability matrix $M$ of size $|\mathbb{S}| \times |\mathbb{S}|$. The expression for generating the values inside $M$ is highly verbose, however to provide the reader some intuition on how it is build, we given an example. Suppose the system is at state $\{50, 50\}$. Then, the system can only move to states $\{49, 51\}$, $\{51, 49\}$, or itself. The probability of moving to $\{49, 51\}$ is the probability of selecting a node that votes value $2$ and having that node switch to value $1$. The probability of staying in place is the probability that any selected node does not achieve the required $\alpha k$ threshold, or it achieves a threshold for its own value. $M$ will be sparse since most states will have only a transition to a small number of states.

% Given any starting state $s \in \mathbb{S}$, the hitting time $\mu$ is the expected number of transitions to reach states $A = \{\{0, |C|\}, \{|C|, 0\}\}$. 
% To calculate the hitting time, we first construct the system of linear equations shown in equation \ref{equation:minimalsolution} for all states in $\mathbb{S}$.

% \begin{equation}
% \label{equation:minimalsolution}
% \begin{cases}
% \mu_{sA} = 0, & \forall s \in A\\
% \mu_{sA} = 1 +\sum_{r\notin A}^{}{p_{sr}\mu_{rA}}, & \forall s \notin A
% \end{cases}
% \end{equation}

% The minimal non-negative solution vector $\mu_{A}~=~(\mu_{sA}, s \in \mathbb{S})$ to the system of linear equations in equation \ref{equation:minimalsolution}, yields the expected number of rounds to reach one of the convergence states. In other words, the solution gives the expected number of rounds for each node before all nodes agree on the same value.

% The convergence latency grows logarithmically with the network size, as shown in Table \ref{table:growth_worst_case}. 
% At 10k nodes, for example, the equal-network split expected time to converge is around 10 rounds. 
% \begin{table}[h!]
% 	\centering
% 	\begin{tabular}{llllll}
% 		Net. Size   & 600    & 1200   & 2400   & 4800   & 9600    \\ \hline
% 		Exp. Conv. & 7.18 & 7.94 & 8.69 & 9.44 & 10.19
% 	\end{tabular}
% 	\caption{Expected number of per-node-iterations to convergence starting at worst-case (equal) network split. Network sizes grow exponentially, whereas worst-case convergence grows logarithmically. $k = 10,\ \alpha=6$.}
% 	\label{table:growth_worst_case}
% \end{table}

\paragraph{Adversarial Progress} 
Without loss of generality, let $\lambda$ be chosen such that the expected frequency of $v_1$ and $v_2$ amongst the $\lambda$ chosen neighbors is nearly the same as $cn(v_1)$ and $cn_(v_2)$. 
In order to prevent progress, the number of adversarial nodes must then be larger than the absolute difference between the total number of honest nodes that vote for $v_1$ and $v_2$. This absolute difference denotes the total number of nodes that the adversary must have in its control in order to maintain an equal split between honest nodes. This adversarial size denotes the minimal adversarial size to prevent convergence in expected logarithmic number of rounds. 

Conversely, we can look at the case when the adversary pushes honest nodes to commit one value, and then equivocates. In this case, As long as the adversary is greater than ($1 - \beta/\lambda$), honest nodes that have not yet committed will no longer be able to commit. Any and all solicitations from any honest node will result in expected $(\lambda-\beta)/\lambda$ or more equivocations, which is insufficient to make progress.

\label{section:analysis}
\subsection{Snowball Safety Analysis}
% \label{subsec:safetyanalysis}
% \subsubsection{Terminology and Definitions}
% \label{subsubsec:termanddef}
% In this subsection, we refresh the reader of some of the old notations and as well introduce new notation, terminology, and definitions. 
%Finally, let $T_i$ and $T_j$ be two conflicting transactions belonging to the same conflict set. 

In order to analyze the safety of our protocol, we turn our focus exclusively towards two transactions of interest, $T_i$ and $T_j$, which belong to the same conflict set. 
Although the system is comprised of many conflicting transactions, we can safely ignore transactions that are not in the ancestry or progeny sub-graph of $T_i$ and $T_j$, since -- by construction -- those transactions are completely independent from $T_i$ and $T_j$ and thus do not contribute to the evolution of preference for either of the transactions of interest. 
Lastly, we note that unless explicitly stated, the analysis is through a ``God's eye'' view of the network. 

In the specification section (S. \ref{subsection:specification}), we introduced the general definition of \textit{preference} for a transaction $T$. 
Using that definition, we construct the notion of \textit{network support} for $T$, denoted as $\mathcal{S}_{u}^{t}(T)$, which represents the fraction of nodes in $\mathcal{N}$ that prefer $T$ at time $t$ as perceived by node $u$. 
To illustrate, suppose that the correct nodes are equally split in preference between $T_i$ and $T_j$. Furthermore, let $\mathcal{B}_{u}^{t}(T_i), \mathcal{B}_{u}^{t}(T_j) \subseteq \mathcal{B}$, be the subsets of the Byzantine nodes that vote $T_i$ and $T_j$ respectively as perceived by node $u$, which are mutually exclusive since according to $u$'s perspective the same Byzantine node cannot prefer two equivocating transactions simultaneously. 
A correct node $u$ would then observe that the network support for $T_{\{i,j\}}$ must be $\mathcal{S}_{u}^{t}(T_{\{i,j\}}) = (|\mathcal{B}_{T_{\{i,j\}}}| + |\mathcal{C}|/2)/|\mathcal{N}|$). 

Lastly, we call a \textit{solicitation} the act of $u$ querying a set of $k$ neighbors, chosen uniformly at random, to discover if they prefer transaction $T_i$. 
Note that necessarily $k \leq |\mathcal{N}|$, but otherwise the choice of size of $k$ is independent of the size of $\mathcal{N}$, as discussed previously.

% \subsubsection{Network Model}
\paragraph{Network Model}
We initially assume that every node has full view of every other node. 
Later, we relax this requirement to allow for looser views. 
Each node maintains a logical round counter (time) that starts at 0 at its initial solicitation and is incremented by one for each solicitation of a child transaction. 
Importantly, we remind that there is no notion of global system rounds, unless explicitly stated.

For simplicity, we assume that each node receives all $k$ responses of a solicitation within the same round. 
Later, we relax this requirement to interleave solicitation responses. 

% \subsubsection{Byzantine Adversary}
% \label{subsec:byzantineadversary}
\paragraph{Byzantine Adversary}
The adversary, whose nodes are in set $\mathcal{B}$, is round-adaptive and can both read all messages and view the state of all nodes in the network.
Round-adaptive means that the adversary can choose a new strategy for each of its nodes after seeing the messages exchanged by correct nodes.
In other words, whenever a correct node solicits its neighbors, the adversary can correspondingly instruct nodes under its ownership before the correct node has the chance to receive any responses. 
Such an adversary is only prohibited from modifying the internal state of a correct node and the in-transit responses between any two correct nodes. 

\subsubsection{Analysis}
\label{subsec:analysis}
% \paragraph{Statistical Errors and Parameters}
% We begin the analysis by first extracting some statistical bounds on protocol parameters. 
% We extract these bounds by isolating a single correct node $u$, and analyzing the results of a single isolated network polling experiment. Basically, we freeze the network at some specific point in time $t$ and then compute the statistical errors between two nodes $u$ and $v$. 

% For notational ease, we represent $\mathcal{S}_{u}^{t}(T_i)$ as $\mathcal{S}'$. 
% Let $\mathcal{H}_{N, \mathcal{S}'}^k \rightarrow [0, k] \in \mathbb{N}$ be a random variable which represents the total count of the $k$ randomly chosen neighbors that prefer transaction $T_i$ at round $t$ as queried by $u$. $\mathcal{H}$ is parameterized by the sample size $k$, the network $\mathcal{N}$, and the network support of $T_i$, $\mathcal{S}'$. For some constant $1/2 \leq \alpha \leq 1$, we are interested in the probability that a majority or more, $\alpha k \in \mathbb{N}$, of the sampled $k$ neighbors prefer $T_i$. The probability can be calculated as follows, 
% \begin{equation}
% P(\mathcal{H}_{\mathcal{N}, \mathcal{S}'}^k \geq \alpha k) = \sum_{j = \alpha k}^{k} \frac{{\mathcal{S}'|\mathcal{N}| \choose j}{|\mathcal{N}| - \mathcal{S}'|\mathcal{N}| \choose k - j}}{{|\mathcal{N}| \choose k}}
% \label{eq:hypergeometric}
% \end{equation}
% where the expected value of $\mathcal{H}_{\mathcal{N}, \mathcal{S}'}^k$ is exactly $k\mathcal{S}'$. From now on, if $\mathcal{H}_{N, \mathcal{S}'}^k \geq \alpha k$, we say that the solicitation was successful. 
% %Intuitively, the meaning behind this term is that some threshold majority $\alpha k$ of the solicited neighbors indeed support the transaction in question.

% We use the Hoeffding \cite{hoeffding1963probability} inequality to calculate the probabilities of deviation from the expected result of the polling experiment. Hoeffding's tail bounds then show that -- given a fixed constant $\psi$ -- the probability $\mathcal{H}$ deviating by $\psi$ from the expected value is given by, 
% \begin{equation}
% \begin{split}
%     P(\mathcal{H}_{N, \mathcal{S}'}^k \leq (\mathcal{S}'-\psi)k) %&\leq e^{-k\mathcal{D}(\mathcal{S}'-\psi, \mathcal{S}')} %\\
%     %&
%     \leq e^{-2\psi^2k}
% \end{split}
% \end{equation}
% % where $\mathcal{D}(\mathcal{S}'-\psi, \mathcal{S}')$ is the Kullback-Leibler divergence, measured as
% % \begin{equation}
% % \begin{split}
% %     \mathcal{D}(\mathcal{S}'-\psi, \mathcal{S}') &= (\mathcal{S}'-\psi) \log (\frac{\mathcal{S}'-\psi}{\mathcal{S}'}) \\
% %     &+ (1 - \mathcal{S}' + \psi) \log \frac{1 - \mathcal{S}' + \psi}{1 - \mathcal{S}'}
% % \end{split}
% % \end{equation}
% The very first thing to notice is that the probabilities are independent of network size, meaning that network size doesn't affect the performance of the protocol. 

% The second thing to notice is that the the upper bound $e^{-2\psi^2k}$ indicates that the probability of success of a solicitation is an inverse exponential parametrized by the sample size $k$. 
% For $k$, every +1 increase means an \textit{exponential decrease} in network view error.

% The third and last thing to notice is the implication for the value $\psi$, which has a quadratic effect on the exponential decrease in network view error. The network split amongst the correct nodes that maximizes the tail bound probability is exactly when half of the correct nodes are partitioned to initially prefer $T_i$ and half to initially prefer $T_j$. If the Byzantine nodes partition the network at some other ratio, the probability the Byzantine adversary successfully forces $u$ to prefer $T_i$ and $v$ to prefer $T_j$ for one solicitation is suboptimal. However, although this conclusion is correct over a single polling experiment, it may not hold over multiple experiments. This is because it would need to account for changes in the underlying graph structure. To that end, we now begin to analyze the protocol as it evolves over time. 

% % The implication of this result is that the optimal strategy for the Byzantine nodes is to minimize the deviation of $\psi$ (i.e. $\psi, k \rightarrow 0$), by splitting the network equally into two conflicting halves. 

% %The structure of the dag confers an important property. 
% %Due to the invariant imposed by the structure of the dag which states that every transaction on the path to a preferred child must be preferred in turn, every successful solicitation of a transaction implies a successful solicitation of its parent. 
% % Let $T' \xleftarrow{*} T$. At any time $t$, we necessarily have 
% % \begin{equation}
% % P(\mathcal{H}_{N, \mathcal{S}_{u}^{t}(T')}^k \geq \alpha k) \geq P(\mathcal{H}_{N, \mathcal{S}_{u}^{t}(T)}^k \geq \alpha k)
% % \end{equation}
% % We can now substitute the net total solicitations of the child transactions with an equivalent set of repeated solicitations for the parent transaction. 
% % This simplification allows us to focus solely on $T_i$, and safely ignore all other transactions except direct ancestors of $T_i$. 

% % Let $\mathcal{P}_b$ = $\{T_i, T_j\}$ be a set of two conflicting transactions. 
% % Let $u, v \in \mathcal{C}$ be any two correct nodes, and let $c_{\{u, v\}}(T_{\{i,j\}}, n)$ represent the confidence (i.e. the number of successful solicitations) for each of the transactions by each of the two correct nodes after sampling $n$ children transactions at rounds $t_0, t_1, \dots, t_n$, respectively. 

% % The expectation of the confidence of transaction $T_i$ after $n$ solicitations is equal to the probability of a successful solicitation for $T_i$ summed independently over every one of the $n$ experiments. More precisely, 
% % \begin{equation}
% % \begin{split}
% %     \mathbb{E}[c_{u}(T_{i}, n)] &=\ \sum_{j = 0}^{n}P(\mathcal{H}_{N, \mathcal{S}_{u}^{t_j}(T_i)}^k \geq \alpha k) \\
% % \end{split}
% % \end{equation}
\paragraph{Evolution Over Time}
The Byzantine nodes have the freedom to attack the system using any strategy. 
In order to maximize damage, the Byzantine nodes must pick the path of execution that ensures that the confidence of the two equivocating transactions is maximized between two correct nodes.
The adversary has access to a large set of attack options. On the one extreme end, the adversary may launch a ``bifurcation attack'', where the attacker equivocates at the very beginning and attempts to split the network equally in half, hoping that part of the network slowly prefers one transaction and the other half prefers the other. On the other extreme end, the adversary can launch a ``double-spend'' attack, where the adversary behaves correctly at the beginning, but after some large amount of time equivocates. 

% To calculate these expectations, and consequently define the most damaging Byzantine strategy, we must first extract some tail bounds on $\mathcal{H}$. 
%Figure \ref{fig:hypersplits} shows the probability of a single successful experiment over various network splits. 
%The probability of a single successful iteration decreases poly-exponentially with increasing difference between $\mathcal{S}N$ and $\alpha k$. 
% The most relevant tail bound can be extracted from Hoeffding \cite{hoeffding1963probability}. Given a network support $\mathcal{S}'$, the expected value of $\mathcal{H}_{N, \mathcal{S}'}^k$ is exactly $k \mathcal{S}'$. Hoeffding's inequality then shows that -- given a fixed constant $\psi$ -- the probability $\mathcal{H}$ deviating by $\psi$ from the expected value is given by, 
% \begin{equation}
% \begin{split}
%     P(\mathcal{H}_{N, \mathcal{S}'}^k \leq (\mathcal{S}'-\psi)k) %&\leq e^{-k\mathcal{D}(\mathcal{S}'-\psi, \mathcal{S}')} %\\
%     %&
%     \leq e^{-2\psi^2k}
% \end{split}
% \end{equation}
% % where $\mathcal{D}(\mathcal{S}'-\psi, \mathcal{S}')$ is the Kullback-Leibler divergence, measured as
% % \begin{equation}
% % \begin{split}
% %     \mathcal{D}(\mathcal{S}'-\psi, \mathcal{S}') &= (\mathcal{S}'-\psi) \log (\frac{\mathcal{S}'-\psi}{\mathcal{S}'}) \\
% %     &+ (1 - \mathcal{S}' + \psi) \log \frac{1 - \mathcal{S}' + \psi}{1 - \mathcal{S}'}
% % \end{split}
% % \end{equation}
% The very first thing to notice is that the probabilities are independent of network size, and are only a function of the sampled neighbor size $k$. This means that the network size doesn't affect performance of the protocol.

% The second thing to notice is that the the upper bound $e^{-2\psi^2k}$ indicates that the probability of success of a solicitation is an inverse exponential parametrized by the squared value of $\psi$. 
% The implication of this result is that the optimal strategy for the Byzantine nodes is to minimize the deviation of $\psi$ (i.e. $\psi, k \rightarrow 0$), by splitting the network equally into two conflicting halves. 
%Correct nodes can be fooled by Byzantine nodes by tuning parameters such that $e^{-2\psi^2k}$ is maximized. 
%This occurs when the deviation and sample size approach zero (i.e. $\psi, k \rightarrow 0$). 
% Since the Byzantine nodes are limited in their network presence, the most damaging strategy must necessarily be when all correct nodes are equally split. 

We start calculating the evolution of confidence between $T_i$ and $T_j$ by first computing the network split between the two transactions without introducing any children transactions. Let $T_*$.\texttt{sum} be the total sum of all chits for transaction $T_*$ amongst all correct nodes in the network. Let $\mathcal{C}_1$ be the subset of correct nodes that prefer $T_i$ at time $t = 0$, and $\mathcal{C}_2$ the corresponding set for $T_j$. Lastly, let $\mathcal{Z}_1$ be the subset of correct nodes that the Byzantine nodes have chosen to force to prefer $T_i$, and $\mathcal{Z}_2$ be the corresponding set of nodes for $T_j$. At $t = 1$ (the base case), the we can compute the new values of $T_*$.\texttt{sum} as follows:

\begin{equation}
    \begin{split}
        & T_1.\text{\texttt{sum}} = 0;\ T_2.\text{\texttt{sum}} = 0;\\
        t_1:\ \ \ &\gamma_{1}^{t_1} \leftarrow \frac{\mathcal{Z}_1}{\mathcal{C}} P(\mathcal{H}(\mathcal{N}, \mathcal{C}_1 + \mathcal{B}, k, \alpha) \geq \alpha k)
        % = \sum_{i = \alpha}^{k} {k \choose i}\bigg(\frac{\mathcal{C}_1 + \mathcal{B}}{\mathcal{N}}\bigg)^i \bigg(1 - \frac{\mathcal{C}_1 + \mathcal{B}}{\mathcal{N}}\bigg)^{k - i}
        \\
        & \gamma_{2}^{t_1} \leftarrow \frac{\mathcal{Z}_2}{\mathcal{C}} P(\mathcal{H}(\mathcal{N}, \mathcal{C}_1, k, \alpha) \geq \alpha k) 
        %= \sum_{i = \alpha}^{k} {k \choose i}\bigg(\frac{\mathcal{C}_1}{\mathcal{N}}\bigg)^i \bigg(1 - \frac{\mathcal{C}_1}{\mathcal{N}}\bigg)^{k - i}
        \\
        & T_1.\text{\texttt{sum}} = T_1.\text{\texttt{sum}} + \gamma_{1}^{t_1} + \gamma_{2}^{t_1}\\
        &\xi_{1}^{t_1} \leftarrow \frac{\mathcal{Z}_1}{\mathcal{C}} P(\mathcal{H}(\mathcal{N}, \mathcal{C}_2, k, \alpha) \geq \alpha k)\\
        & \xi_{2}^{t_1} \leftarrow \frac{\mathcal{Z}_2}{\mathcal{C}} P(\mathcal{H}(\mathcal{N}, \mathcal{C}_2 + \mathcal{B}, k, \alpha) \geq \alpha k)\\
        & T_2.\text{\texttt{sum}} = T_2.\text{\texttt{sum}} + \xi_{1}^{t_1} + \xi_{2}^{t_1}\\
    \end{split}
\end{equation}

In other words, the new expected value of $T_1$.\texttt{sum} after a single time-step is the probability that a correct node in $\mathcal{Z}_1$ is chosen and that node successfully samples at least $\alpha k$ neighbors that also prefer $T_i$ plus the probability that a correct node in $\mathcal{Z}_2$ is chosen and that node successfully samples at least $\alpha k$ neighbors that also prefer $T_i$. In the next time-step, we must include the newly-updated transaction preference sums as part of the computation. For the rest of the time-steps, we compute as follows:

\begin{equation}
    \begin{split}
        t_2:\ \ \ &\gamma_{1}^{t_2} \leftarrow \frac{\mathcal{Z}_1}{\mathcal{C}} P(\mathcal{H}(\mathcal{N}, \mathcal{C}_1 + \mathcal{B} + \gamma_{2}^{t_1} - \xi_{1}^{t_1}, k, \alpha) \\&\geq \alpha k)\\
        & \gamma_{2}^{t_2} \leftarrow \frac{\mathcal{Z}_2}{\mathcal{C}} P(\mathcal{H}(\mathcal{N}, \mathcal{C}_1 + \gamma_{2}^{t_1} - \xi_{1}^{t_1}, k, \alpha) \geq \alpha k)\\
        & T_1.\text{\texttt{sum}} = T_1.\text{\texttt{sum}} + \gamma_{1}^{t_2} + \gamma_{2}^{t_2}\\
        &\xi_{1}^{t_2} \leftarrow \frac{\mathcal{Z}_1}{\mathcal{C}} P(\mathcal{H}(\mathcal{N}, \mathcal{C}_2 + \xi_{1}^{t_1} - \gamma_{2}^{t_1}, k, \alpha) \geq \alpha k)\\
        & \xi_{2}^{t_2} \leftarrow \frac{\mathcal{Z}_2}{\mathcal{C}} P(\mathcal{H}(\mathcal{N}, \mathcal{C}_2 + \mathcal{B} + \xi_{1}^{t_1} - \gamma_{2}^{t_1}, k, \alpha) \geq \alpha k)\\
        & T_2.\text{\texttt{sum}} = T_2.\text{\texttt{sum}} + \xi_{1}^{t_2} + \xi_{2}^{t_2}\\
        t_3:\ \ \ &\gamma_{1}^{t_3} \leftarrow \frac{\mathcal{Z}_1}{\mathcal{C}} P(\mathcal{H}(\mathcal{N}, \mathcal{C}_1 + \mathcal{B} + \gamma_{2}^{t_1} + \gamma_{2}^{t_2} - \xi_{1}^{t_1} - \xi_{1}^{t_2}, k, \alpha) \geq \alpha k)\\
        & \gamma_{2}^{t_3} \leftarrow \frac{\mathcal{Z}_2}{\mathcal{C}} P(\mathcal{H}(\mathcal{N}, \mathcal{C}_1  + \gamma_{2}^{t_1} + \gamma_{2}^{t_2} - \xi_{1}^{t_1} - \xi_{1}^{t_2}, k, \alpha) \geq \alpha k)\\
        & T_1.\text{\texttt{sum}} = T_1.\text{\texttt{sum}} + \gamma_{1}^{t_3} + \gamma_{2}^{t_3}\\
        &\xi_{1}^{t_3} \leftarrow \frac{\mathcal{Z}_1}{\mathcal{C}} P(\mathcal{H}(\mathcal{N}, \mathcal{C}_2 + \xi_{1}^{t_1} + \xi_{1}^{t_2} - \gamma_{2}^{t_1} - \gamma_{2}^{t_2}, k, \alpha) \geq \alpha k)\\
        & \xi_{2}^{t_3} \leftarrow \frac{\mathcal{Z}_2}{\mathcal{C}} P(\mathcal{H}(\mathcal{N}, \mathcal{C}_2 + \mathcal{B} + \xi_{1}^{t_1} + \xi_{1}^{t_2} - \gamma_{2}^{t_1} - \gamma_{2}^{t_2}, k, \alpha) \geq \alpha k)\\
        & T_2.\text{\texttt{sum}} = T_2.\text{\texttt{sum}} + \xi_{1}^{t_3} + \xi_{2}^{t_3}\\
        t_4:\ \ \ & \dots
    \end{split}
\end{equation}

Calculating this complex expression, we arrive at the following results shown in Figures \ref{fig:variousalpha}, \ref{fig:variousk}, and \ref{fig:variousb}.

\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{./various_alpha.png}
\caption{Various $\alpha$}
\label{fig:variousalpha}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{./various_k.png}
\caption{Various $k$}
\label{fig:variousk}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{./various_b.png}
\caption{Various $\mathcal{B}$}
\label{fig:variousb}
\end{figure}

$<<$TODO: DISCUSS IMPLICATIONS OF THE GRAPH, AND HOW THEY SUPPORT PRIOR CLAIMS.$>>$

At $t_0$, the Byzantine nodes partitioned the correct nodes according to some strategy, and we computed the expected outcomes of the network preferences after all correct nodes had a chance to poll. We now continue computing the evolution of the preferences in the network by introducing children transactions. For simplicity, we first assume that the children transactions all belong to partitions of size one, even if the children transactions are generated by Byzantine nodes.

Due to the invariant imposed by the structure of the dag which states that every transaction on the path to a preferred child must be preferred in turn, every successful solicitation of a transaction implies a successful solicitation of its parent. Moreover, and more importantly, the network support for every immediate child transaction is exactly equal to the probability of the parent being preferred. 
Let $T' \xleftarrow{} T$. At any time $t$, we necessarily have 
\begin{equation}
P(\mathcal{H}_{N, \mathcal{S}_{u}^{t}(T')}^k \geq \alpha k) \geq P(\mathcal{H}_{N, \mathcal{S}_{u}^{t}(T)}^k \geq \alpha k)
\end{equation}
and, more importantly, the 
\begin{equation}
\mathcal{S}_{u}^{t_b}(T) = \mathbb{E}[\mathcal{H}_{N, \mathcal{S}_{u}^{t_a}(T')}^k]/k
\end{equation}
where $t_b$ is larger than $t_a$. 
The expectation of confidence between two conflicting transaction in a permanently split network after $n$ rounds is then
\begin{equation}
    \begin{split}
        \mathbb{E}[c_{u}(T_{i}, n)] &=\ \mathbb{E}[c_{v}(T_{j}, n)]\\
         &=\ nP(\mathcal{H}_{\mathcal{N}, |\mathcal{H}|/2 + |\mathcal{B}|}^k \geq \alpha k)\\
\end{split}
\end{equation}

Before moving on, we can now extract some numerical values. 
Let $|\mathcal{N}| = 10000$, where 25\% of nodes are Byzantine.
Let half of the correct nodes prefer $T_i$ such that $d(T_i) = 1$ and $d(T_j) = 0$, and the other half prefer $T_j$ such that $d(T_i) = 0$ and $d(T_j) = 1$.
Let $u$ be a correct node that prefers $T_i$ and $v$ a correct node that prefers $T_j$.
Let $\alpha k$ = 180, and $k$ = 200. 
Then, 
\begin{equation}
    \begin{split}
    P(\mathcal{H}_{\mathcal{N}, \mathcal{S}_{u}^{t_1}(T_i)}^k \geq \alpha k) &= P(\mathcal{H}_{\mathcal{N}, \mathcal{S}_{v}^{t_1}(T_j)}^k \geq \alpha k)\\
    &= 5.616\times10^{-19}
    \end{split}
\end{equation}
as calculated from equation \ref{eq:hypergeometric}. 
If compounded over all nodes in the network, then the probability that any two nodes from the two preferrence subsets successfully increase confidence in their respective preference is $4.435\times10^{-30}$. 
% Other splits are shown in Figure \ref{fig:hypersplits}. 
%The probability that specifically $u$ and $v$ prefer $T_i$ and $T_j$ for only a preference difference of 1 is $3.154\times10^{-37}$. 
%If we compound over all pairs of partitioned correct nodes, then the probability increases to $4.435\times10^{-30}$. 
Notice that this is for a single round. If we assume a throughput of 1000 solicitations/second, then the probability of success over a second increases to $4.435\times10^{-27}$. Therefore, the expected time before any two correct nodes prefer two equivocating transactions can be calculated through the mean of the geometric distribution and is equal to $2.25\times10^{26}$ seconds, or about $7.14\times10^{18}$ years.

Notice that the calculation above is the optimal probability. Other splits in network result in far lower probabilities and far longer times. Furthermore, notice that the above Byzantine attack assumes that Byzantine nodes can arbitrarily generate transactions \textit{at will}. In reality, simple anti-transaction-flooding measures would severely cripple the Byzantine adversary. 

Let's break down the intuition of the results in our analysis. 
The tail bounds indicate that as long as a reasonably large $k$ sample size is picked, the only way for the Byzantine nodes to fool any correct node is to actually build enough network confidence for the transaction. 
The threshold $\alpha$ can be chosen as a function of the Byzantine size, where the higher the Byzantine presence, the larger the threshold should be set. 

The consequence of a higher $\alpha$, however, is that it is possible for the Byzantine nodes to deny service to the network. Since liveness is decoupled from safety, we later introduce non-protocol specific mechanisms to thwart such behavior, ensuring that rogue transactions die out quickly and virtuous transactions get accepted quickly.

\subsubsection{Network View}
The analysis up to now assumes that the network view is fully consistent among all nodes. 
In any real open distributed system, such an assumption invariably breaks downs. 
Therefore, we must quantify the amount of tolerance in network view discrepancy between any two correct nodes. 

Safety may be violated using a subnetwork partition attack. 
The Byzantine nodes are able to partition the network into several subnetworks such that each subnetwork shares only some set of correct nodes. 
To make this clear, let $\mathcal{E}_{1}, \mathcal{E}_{2} \subset \mathcal{N}$, where $\mathcal{E}_1 \cup \mathcal{E}_2 = \mathcal{N}$, be two subsets of the entire network of nodes, where all members of each subset have -- at minimum -- all other members in the same subset in their view. 
Lastly, let the nodes in the intersection $\mathcal{E}_1 \cap \mathcal{E}_2$ have a view of all nodes in $\mathcal{E}_1$ and $\mathcal{E}_2$. 
We can then view each subnetwork independently of each other, and apply the same analysis as before. The difference, however, is that the network of nodes from the perspective of each subnetwork is not $\mathcal{N}$, but rather just $\mathcal{E}_*$. Therefore, if the Byzantine presence with a fully consistent view was only $\mathcal{B}/\mathcal{N}$, it now becomes $\mathcal{B}/\mathcal{E}_*$. In the worst case scenario, if $|\mathcal{E}_1 \cap \mathcal{E}_2| < (k - \alpha k)$, then safety can be violated without any Byzantine presence. However, in practice, although churn exists, such large network partition is difficult to achieve. 

In later sections, we introduce the Snowball network overlay protocol, which guarantees with high probability that the network doesn't suffer from large partitioning. 

% \begin{figure}
% \centering
% \includegraphics[width=\linewidth]{./hypersplits.pdf}
% \caption{Probability of single successful sample over different network splits.}
% \label{fig:hypersplits}
% \end{figure}
\end{comment}


==> rvr_todo <==
- Section 3.1: perhaps rename “Safety Analysis of Slush”
- lemma 3 seems awkwardly worded, with \phi’ being unbounded.  Also, it seems unlikely unless “whp” is added.
- pg 7: targetstate —> target state
	- Kevin: Done.
- pg 7: and we iteratively solve —> we iteratively solve
	- Kevin: Done.
- Figure 9: what’s \eps?  Shouldn’t we know this?
	- Kevin: \epsilon is discussed previously in the paper.
- Figures 10 and 11 are out of order wrt text
- pg 8: Finally, —> remove
	- Kevin: Done
- Section 3.1: take home message is unclear. Add last paragraph
- Section 3.2: perhaps rename “Safety Analysis of Snowflake”
- pg 8: color(u.cnt) —> color (u.cnt)
- pg 9: term “irreversible” used before it’s defined
- pg 9: “one crucial condition”: what condition are you referring to?
- pg 9: for some upper bound \phi: \phi is the number of steps, not an upper bound
- pg 9: that then models —> that models
- Theorem 6: proof needs more explanation.  What do you mean by differential?
- Figure 13 caption: Snowflake/Snowball —> Snowflake and Snowball
- pg 9: “For the system to guarantee safety, …”: why?
- pg 9: That is, we need to ensure that …: I have no clue where Eq. 14 comes from or what it means
- pg 9: I don’t understand the paragraph that follows either.  Is IsAccepted still defined the same way?
- Section 3.2: in the end, it’s not clear how the analysis relates to the adversarial game defined in the section.
- Section 3.3: perhaps rename “Safety Analysis of Snowball”
- it would be good to know why we analyzed Snowflake, which is, we’re going to show that if Snowflake is safe, then so is Snowball
- pg 10: definition of “prefers” doesn’t say anything about the situation where a node has equal confidence in both colors
- pg 10: how do Byzantine nodes in Snowball do a “setup” that cause some correct nodes to accept R.  Why “some” and not just “one”?
- pg 10: why is it that if a correct node accepts R, then s_{c/2+\Delta} correct nodes “vote” for R?  Why s_{c/2+\Delta} and not c/2+\Delta?  What does it mean to vote exactly?
- pg 11: is “commit point” same as “phase shift point”?  Is “at commitment” the same as well?
- pg 11: prove (R1): what’s R1?
- Theorem 7: I can’t follow the proof
- Section 3.4: perhaps rename “Safety Analysis of Avalanche”
- pg 12: I don’t know where the right hand side of Eq. 22 came from


==> sections/other-crypto.tex <==
\subsection{Snowball vs. Blockchain}
Informally speaking, Nakamoto consensus achieved by the Blockchain
algorithm, is a process where the whole system synchronizes their replicated
log by creating a large time delay upon each generation of a block. The
Blockchain system is leaderless because there is no notion of elected leader
that could control the content of multiple slots on the log. However, the peer who is lucky enough
to come up with the block containing a proper nonce will take over the
ownership of the slot, and thus becomes a conceptual temporary ``leader''
only for the slot.  This analogy to traditional BFT reveals the
fundamental inefficiency in Nakamoto consensus, where each commonly accepted
block can be viewed as the outcome of a one-time leader election, the creator
of the block loses leadership immediately after establishment of the block.

There have been work on improving the performance by explicitly stating and
extending the leadership to several slots, such as Bitcoin-NG and Thunderella.
But this makes the protocol leader-based, and may suffer from the issues of
having a single leader in an Internet-scale network environment.

On the other hand, Nakamoto consensus was originally used for Bitcoin, a
peer-to-peer electronic cash system. So each block usually contains hundreds or
thousands of transactions that are mutually compatible (no double spending of
money), and there exists another separated logic, UTXO (Unspent Transaction
Output) graph that is made of all transactions to represent the actual state of
the cash system. On a UTXO graph, a transaction has multiple inputs and
outputs. A valid transaction will provide with signature proofs for all the
inputs that correspond and consume some outputs from some transactions prior in
history, and then offer some dangling unspent outputs which could be taken as
inputs in the future by subsequent transactions. The whole UTXO graph is valid
only if there does not exist two or more transactions that take the same input,
which is usually called a ``double spend''. With that being said,
Nakamoto consensus provides with more power than that is required for
maintaining a double-spend-free UTXO graph, because Blockchain ensures all transactions are
\emph{linearly} ordered, while a valid UTXO graph used for ledger does not
require such linear ordering. For example, suppose there are two transactions
A, B that both have only one input taken from one of the two outputs from
transaction C. So using Blockchain, eventually only a specific linear ordering
of A, B and C will be accepted, which might be unnecessary because both C, A, B
and C, B, A are valid orderings as A and B are independent. The only
necessary dependencies are all exactly captured by UTXO graph itself.

This leads to two possible paths of research: to fully utilize the ability
of keeping a linear log as in state machine replication so Nakamoto consensus is
not wasted, or to construct another weaker consensus that only resolves double
spends, not capable of keeping a linear log but just fits the need for an
electronic cash system. One well-known system for the first approach is
Ethereum, a decentralized application platform that makes use of the linear log
to certify executions and interactions of smart contract logic. The second approach motivates us
to Snowball.




==> sections/protocol.tex <==
Snowball is a leaderless, multi-decree, probabilistic consensus protocol that makes
use of sub-sampled voting. It entangles voting results to render the process
more efficient than independently deciding on each item alone. We first provide
the intuition behind the protocol informally, then present the formal protocol
specification, followed by a proof of safety and discussion on liveness for virtuous
transactions.

\subsection{Intuition}

The protocol operates by building a directed acyclic graph (DAG) of all known transactions.
This DAG is rooted at a protocol-defined \emph{genesis} transaction shared by all nodes.
Each transaction is represented as a vertex in the DAG.
When a transaction is created, it names one or more \emph{parent transactions}, which point to already accepted vertices in the DAG.
The parent-child relationships encoded in the DAG do not correspond to application-specific structure; for instance, a child vertex need not spend or have any relationship with the funds received in the parent transaction.
These relationships exist solely to entangle and enforce the fate of previous decisions made by the system.
For each vertex in the resulting DAG, there exists a static \emph{ancestor set} that contains all transactions reachable via parent edges back in history, and a \emph{progeny} that recursively includes all children transactions and their offspring.

The central challenge in Snowball is to choose among a set of conflicting transactions.
This notion of conflict in Snowball is application-defined.
In a cryptocurrency application, transactions that spend the same funds (\emph{double-spends}) form a \emph{conflict set}, out of which only a single one can be accepted.
Note that the graph structure of transactions that depend on each other, also known as the UTXO graph, is completely independent of the DAG that Snowball maintains. As a result, any two vertices may be in conflict.
Figure~\ref{fig:dag-conflicting-set} shows an example.

\begin{center}
    \input{figures/dag-conflicting-set}
    \captionof{figure}{The DAG structure in Snowball.  Shaded groups of transactions indicate \emph{conflict sets}---transactions that are conflicting.}\label{fig:dag-conflicting-set}
\end{center}

Snowball makes its choice of an accepted transaction from a conflict set using a novel voting protocol.
%Snowball makes its choice of an accepted transaction from a conflict set using a meta-stable, intertwined voting protocol.
The insight behind this protocol is for the correct nodes in the system to topple over, or ``roll snowball'', towards a system-wide decision.
Of course, the FLP impossibility result~\cite{fischer1985impossibility}
implies that there will be a path where the system remains perfectly in balance among a set of conflicting options, but remaining in this state for long periods of time are probabilistically unlikely.
The decision protocol is designed to amplify and reinforce random perturbations encountered during sampling, leading to a decision.

Snowball's voting protocol takes advantage of the DAG structure that the system maintains.
Specifically, every node independently measures the amount of network-wide support for every new transaction it encounters by sampling a subset of its peers and querying them for whether they could accept this transaction, and by extension, its ancestors.
This is, in effect, a one-time sub-sampled vote on this transaction.
If more than a threshold of responders vote positively, this transaction collects a \emph{chit}.
Nodes associate a second metric, called \emph{confidence}, with every transaction, where confidence is the sum of chits in the progeny of that transaction.
In a bit of seemingly circular logic, nodes vote positively on transactions only when they have high confidence for all transactions in the ancestor set.
In practice, the circulatory is broken by an initial arbitrary preference for first-seen transactions, and the genesis transaction as a common ancestor for bootstrapping.

Overall, %YYY
by repetitive voting that yields chits building up confidence,
guiding future voting towards the same direction, a positive
feedback is rapidly established once a perturbation is detected, so the network
topples towards the same decision in collaboration of all correct nodes, which
results in a protocol with probabilistic, efficient guarantee.

\subsection{Specification}
\label{subsection:specification}

% TODO add definitions on "what is compatible", "what is a conflict set". Specification should stand on its own without the intuition 

% TODO Remove the conflict set stuff
Let the system be comprised by a set of nodes $\mathcal{N}$, where each node is an independent processing unit that stores some local state. 
All nodes are connected to each other through a network and communicate by exchanging messages.
The local state can be modified by executing transactions
% -- denoted by $T_*$ --
that represent special types of messages that encode a sequence of deterministic commands.

Each node $u \in \mathcal{N}$ keeps track of all transactions it has learned about in set $\mathcal{T}_u$. 
This set is partitioned into mutually exclusive \emph{conflict sets},
% subsets, denoted by $\mathcal{P}_*$,
where each transaction in $\mathcal{T}_u$ belongs to exactly one conflict set. 
Transactions are determined to be conflicting based on a deterministic and known function which is run by every node. 
We denote by $\mathcal{P}_T$ the conflict set that transaction $T$ is in.
If $T_i$ and $T_j$ are conflicting transactions, then
$\mathcal{P}_{T_i} = \mathcal{P}_{T_j}$.
% Let $T_i$ and $T_j$ be two transactions that belong in the same conflict set $\mathcal{P}$.
% subset of $\mathcal{T}_u$, i.e. $T_i, T_j \in \mathcal{P}_b$. 
% We then refer to $T_i$ and $T_j$ as conflicting transactions, and to $\mathcal{P}$ as the partition of $T_i$ and $T_j$. 
% For notational ease, we refer to $\mathcal{P}$ as $\mathcal{P}_{T_i}$ or $\mathcal{P}_{T_j}$. 
% The index of the latter two partitions intuitively refers to the partition that $T_i$ and $T_j$ belong both belong to, respectively, even though ultimately both transactions belong to the same partition $\mathcal{P}_b$.

%All transactions in $\mathcal{T}$ are partitioned by some pre-defined equivalence relation into disjoint conflict sets.
Part of the information encoded in the each transaction $T$ are links to other transactions, called parent transactions. 
We write $T' \gets T$ if $T$ has a parent link to a transaction $T'$.
Additionally, the ``$\stackrel{*}{\gets}$''-relation is the reflexive transitive closure of the ``$\gets$''-relation; 
namely, if $T' \stackrel{*}{\gets} T$, then there exists a path from $T$ to $T'$. 
These links, when aggregated amongst all known transactions, generate a DAG. 
Additionally, every transaction $T$ has associated with it a binary value chit, $c_T$, that stores the results of a one time vote.
The chit is not encoded in the transaction, but rather is computed as part of a voting mechanism. 
Based on this DAG, each node can compute a confidence value, $d(T)$, that sums up the number of chits in $T$'s progeny as follows:
\[ d(T) = \sum_{T' \in \mathcal{T}, T \stackrel{*}{\gets} T'}c_{T'}.\]

Each node $u$ maintains its own local list of known nodes $\mathcal{N}_u \subseteq \mathcal{N}$ that comprise the system.
For simplicity of exposition, we assume that all nodes share the same view, i.e. $\mathcal{N}_u = \mathcal{N}$, and later discuss how this assumption can be relaxed. 
% TODO talk to ted and ask how to rephrase this. "the data structure" is unclear, and so is immutability
Note that although $\mathcal{T}$ can vary between nodes, the inferred DAG will always be compatible between any pair of nodes.
% , because the data structure is immutable.
Specifically, if $T' \gets T$, transaction $T$ has a parent link to $T'$, then every node in the system will eventually see the same relation $T' \gets T$; on the other hand, if $T' \cancel{\gets} T$, transaction $T'$ is not a parent of $T$, then no nodes will end up with $T' \gets T$.
%Here, notation ``$T' \gets T$'' means $T'$ is one of $T$'s immediate parents, and
%``$\stackrel{*}{\gets}$''-relation is the reflexive transitive closure of ``$\gets$''-relation; namely,
%if $T' \stackrel{*}{\gets} T$, there exists a path from $T$ to $T'$. Specially, ``$T \stackrel{*}{\gets} T$''.

Each node implements an event-driven state machine, centered around a ``poll'' event which serves both to solicit votes on a transaction and, simultaneously, notify other nodes of the existence of the newly discovered transaction.

When node $u$ discovers a transaction $T$ for the first time, through a poll message it receives, it will start a one-time polling process by sampling $k$ other nodes uniformly at random.
This polling process starts by adding $T$ to $\mathcal{T}_u$, initializing the chit value $c_T$ to $0$, determining the set of conflicting transactions $\mathcal{P}_T$, and then sending a recursive poll message for $T$ to the selected $k$ sample peers.

When a node receives a poll solicitation for a transaction $T$ that it has seen before, it votes in support or against $T$.
Votes reflect the suitability of transaction $T$ for acceptance, compared to the acceptance status of other transactions in $T$'s conflict set $\mathcal{P}_T$, recursively applied to all transactions in $T$'s ancestry.
They are computed by checking whether the confidence for $T$ is the highest among competing transactions $\forall T' \in \mathcal{P}_*$.
If every single ancestor of $T$ fulfills this criteria, the transaction is said to be \emph{strongly preferred}, and receives a unit (1) vote. A failure of this criteria at $T$ or any of its ancestors yields a null (0) vote.

Node $u$ will tally the responses it receives, and form an opinion on the suitability of the transaction for acceptance based on voting results.
Specifically, if $k$ responses have been received, it computes a new chit value $c_T$ for transaction $T$.
It sets $c_t$ to 1 if a threshold $\alpha k \in \mathbb{N}$ of the responses were positive, and to 0 otherwise.  Once computed, a chit value is never modified again.
If fewer than $k$ responses are returned, the node will retry by sampling additional nodes until it has acquired a total of $k$ responses.
% sampled uniformly at random.

The above process will yield a labeling of the DAG with chits $c_T$ and associated confidence for each transaction $T$.
Because chit values can only increase (from 0 to 1),
confidence values are monotonically increasing.

\begin{center}
    \input{figures/dag-cd}
    \captionof{figure}{Example of chits and confidence values.  Darker boxes mean transactions with greater confidence values.}\label{fig:dag-cd}
\end{center}

In Figure~\ref{fig:dag-cd}, notation $\langle c_T, d(T)\rangle$ is the pair of voting result
$c_T$ and confidence $d(T)$ tagged to each transaction $T$.  Notice $c_T$ is
immutable after voting, while $d(T)$ is subject to change as the DAG grows.
Given the
voting rule, the system will topple over to a single transaction in each
conflict set.  For example, in set~2, $T_2$ has much larger confidence than
$T_3$ so it will likely be voted $c_{T_2} = 1$ in the future.

%YYY
%what I really want to write here is that there exists some equation X, that gives us the probability that
%T will get reverted. As a probabilistic protocol, we cannot provide a clear commit point. So applications
%can at best decide to commit a transaction when the probability of reversion is low enough for their use.
%In this sense, we are exactly like Nakamoto consensus.
%There should be a function $\gamma$ that gives us the probability of reversion.

Finally, unlike deterministic protocols, Snowball leaves the finalization of a
transaction to the application, by providing a predicate associated with
probabilistic guarantee.  The \textsc{isCommitted} predicate becomes true when $T$ is the
preferred transaction in its conflict set, and the confidence $d(T)$ exceeds
the sum of the confidence for all conflicting transactions by a constant
$\beta$ (XXX change here). As a probabilistic protocol, the truth of this predicate could be flipped, though,
with very low probability depending on the security parameter $\beta$. The
application using Snowball achieves the finality by choosing the appropriate
security parameters that deliver the desired probabilistic bound of safety:
given the observation of \textsc{isCommitted} being true, the
probability of all correct nodes eventually stick to true.

%The Snowball protocol relies on two security parameters $\alpha$ and $\beta$.
%XXX describe alpha and beta, and how they are selected based on desired probability of loss
%XXX if transactions carry monetary amounts, one can bound the actual dollar loss by multiplying
%XXX \gamma with the amount of the transaction.

The final outstanding component of the protocol is transaction generation, specifically, the choice of parents for a newly minted transactions.
We note that this choice does not affect the safety guarantees of the protocol, as discussed later in our analysis in Subsection \ref{subsec:safetyanalysis}. 
%Because for a particular transaction in the DAG, its confidence solely depends on the chits in its own progeny. 
%Moreover, since the \textsc{isCommitted} predicate is determined by the difference of confidence between transactions in the same conflict set, the only thing that matters in affecting the difference is which progeny set future transactions attach them to, rather than the microscopic DAG structure within the progeny sets.
However, parent selection can significantly affect the liveness of certain transactions, where transactions with badly chosen parents can remain stuck, forever unable to accrue the confidence required for commitment. 
In Section~\ref{sec:parent}, we provide three heuristics,
\emph{random}, \emph{frontier}, and \emph{adaptive}, and show that adaptive parent selection leads to good liveness properties that the \textsc{isCommitted} predicate will be probabilistically guaranteed to hold eventually for virtuous transactions.
%YYY what is good liveness?
A virtuous transaction is guaranteed to have a singleton conflict set consisting of just itself.

Figure~\ref{fig:gossipchain-ongen} shows the initialization of
a node's variables as well as what happens when a node learns of a
new transaction.  Section~\ref{sec:parent} discusses parent
selection from $\mathcal{T}$ for new transactions (which does not
affect safety).

\begin{figure}
\begin{center}
\begin{algorithmic}[1]
    \small
    \Procedure{init}{}
        \State $\mathcal{T} \coloneqq \emptyset$ \hspace{1ex}\textrm{// the set of known transactions}
        \State $\mathcal{Q} \coloneqq \emptyset$ \hspace{1ex}\textrm{// the set of polled transactions}
    \EndProcedure
    \Procedure{onGenerateTx}{$\mathrm{data}$}
        \State $\mathrm{edges} \coloneqq \{T' \gets T: T' \in \Call{parentSelection}{\mathcal{T}}\}$
        \State $T \coloneqq \texttt{Tx}(\mathrm{data}, \mathrm{edges})$
        \State $\mathcal{T} \coloneqq \mathcal{T} \cup \{T\}$
    \EndProcedure
    \Procedure{onReceiveTx}{$T$}
        \If{$T \notin \mathcal{T}$}
            \State $\mathcal{P}_T \coloneqq \mathcal{P}_T \cup \{T\}$
            \State $\mathcal{T} \coloneqq \mathcal{T} \cup \{T\}$
            \State $c_T \coloneqq 0$.
        \EndIf
    \EndProcedure
    \captionof{figure}{Transaction generation and bookkeeping.}\label{fig:gossipchain-ongen}
\end{algorithmic}
\end{center}
\end{figure}

% In Figure~\ref{fig:dag-conflicting-set}, there are 9 transactions and 6
% conflict sets. Solid edges represent parent relation and purple area stands for
% conflict set grouping.  Transaction $T_8$ has two parents $T_4$ and $T_5$ while
% the others only have one.

Figure~\ref{fig:gossipchain-main} shows the main loop of the core protocol.
In each iteration, the loop attempts to select a transaction $T$ that has not
yet been polled, but whose ancestors have all been polled.  (If no such
transaction exists, the loop will stall until a new transaction is
added to $\mathcal{T}$.)
The loop then selects $k$ peers and polls those peers.
If more than $\alpha k$ of those peers return a positive response,
the chit value is set to~1.  Then $T$ is added to the set $\mathcal{Q}$
so it will never be polled again by the node.
(The code that selects additional peers if some of the $k$ peers are
unresponsive is omitted for simplicity.)

\begin{figure}
\begin{center}
\small
\begin{algorithmic}[1]
    \Procedure{gossipChain}{}
        \While {\texttt{true}}
            \State \textrm{// select Tx with polled ancestors}
            \State\textrm{find  $T$ that satisfies }%\vspace*{-.6\baselineskip}
            $T \in \mathcal{T} \land T \notin \mathcal{Q}$
            %\begin{align*}\hspace{2ex}
            %    T \in \mathcal{T} &\land T \notin \mathcal{Q} \\
            %            &\land (\forall T', T' \gets T: T' \in \mathcal{Q})
            %\end{align*}
            \State \textrm{// randomly sample from the known nodes}
            \State $\mathcal{K} \coloneqq \texttt{sample}(\mathcal{N}, k)$
            \State $P \coloneqq \sum_{i \in \mathcal{K}}\texttt{poll}(i, T)$
            \If{$P > \alpha\cdot k$}
                \State $c_T \coloneqq 1$
            \EndIf
            \State\textrm{// otherwise, }$c_T$\textrm{ remains 0 forever}
            \State $\mathcal{Q} \coloneqq \mathcal{Q} \cup \{T\}$ \hspace {1ex} \textrm{// mark T as polled}
        \EndWhile
    \EndProcedure
    \captionof{figure}{The main gossip loop.}\label{fig:gossipchain-main}
\end{algorithmic}
\end{center}
\end{figure}

% TODO IMPORTANT The isPreferred must imply that T is polled, but current writing can be not polled. Also, do you do max over only polled transactions? 
\begin{figure}
\begin{center}
\small
\begin{algorithmic}[1]
    \Function{isPreferred}{$T$}
        \State \Return $d(T) = \max_{T' \in \mathcal{P}_T} d(T')$
    \EndFunction
    \Function{isStronglyPreferred}{$T$}
        \State \Return $\forall T'\in\mathcal{T}, T' \stackrel{*}{\gets} T: \Call{isPreferred}{T'}$
    \EndFunction
    \Procedure{onPoll}{$j, T$}
        \State \Call{onReceiveTx}{$T$}
        \If{\Call{isStronglyPreferred}{$T$}}
            \State $\Call{respond}{j, 1}$\hspace{2ex}\textrm{// vote yes}
        \Else
            \State $\Call{respond}{j, 0}$\hspace{2ex}\textrm{// vote no}
        \EndIf
    \EndProcedure
    \captionof{figure}{The voting rule.}\label{fig:gossipchain-onpoll}
\end{algorithmic}
\end{center}
\end{figure}

Figure~\ref{fig:gossipchain-onpoll} shows what happens when a node
receives a poll for a transaction $T$ from a peer $j$.
First it adds $T$ to $\mathcal{T}$, unless it already has it.
Then it determines if $T$ is currently strongly preferred.
If so, the node returns a positive response to peer $j$.
If not, the node returns a negative response.

\begin{figure}
\begin{center}
\begin{algorithmic}[1]
    \small
    \Function{isCommitted}{$T$}
        \State\Return
            \vspace*{-.8\baselineskip}
        \begin{align*}
            \Call{isPreferred}{T} &\land d(T) \\
            &- \sum_{T' \in \mathcal{P}_T, T' \neq T}{d(T')} \ge \beta
        \end{align*}
    \EndFunction
    \captionof{figure}{The commit condition.}\label{fig:gossipchain-diff-commit}
\end{algorithmic}
\end{center}
\end{figure}

Finally, Figure~\ref{fig:gossipchain-diff-commit} shows pseudo-code for
the commit decision for a transaction $T$.

\subsection{Parent Selection}
\label{sec:parent}

The goal of the parent selection policy is to yield a well-structured DAG that maximizes
the likelihood that virtuous transactions will be quickly accepted by the network. While this
policy will not affect the safety of the protocol, it plays a crucial role in determining
the shape and structure of the DAG, and affects liveness.

There are inherent trade-offs in the parent selection policy: selecting well-accepted parents make it
more likely for a transaction to find support, but can lead to vote dilution; as well, selecting more
recent parents at the frontier of the DAG can lead to stuck transactions, as the parents may turn out
to be in conflict and remain unsupported.  In the following discussion, we illustrate this dilemma.
We assume that every transaction will select a small number, $p$, of parents, provided as a protocol parameter.
We focus on the the selection of eligible parent set, from which a subset of size $p$ can be chosen at random.

Perhaps the simplest idea is to mint a fresh transactions with parents picked uniformly at random
among those transactions that are already well-accepted. Specifically, we can adopt the predicate
used in the voting rule to determine eligible parents on which a node would vote positively, as follows:
\[
    \mathcal{E} = \{T: \forall T\in\mathcal{T}, \textsc{isStronglyPreferred}(T)\}.
\]

But this strategy has the drawback that it can suffer from vote dilution and lead to starved transactions.
This heuristic will yield to large sets of eligible parents, consisting mostly of historical, old transactions.
When a node samples the transactions uniformly from $\mathcal{E}$, the resulting DAG
will have large, ever-increasing fan-out. Because new transactions will have scarce progenies,
the voting process will take a long time to build the required confidence on any given new transaction.

In contrast, efforts to reduce fan-out and control the shape of DAG by selecting the recent transactions at
decision frontier suffers from another problem. Most recent transactions will have very small (usually zero) $d$ values,
simply because they do not have enough descendants. Further, their conflict sets may not be well-distributed
and well-known across the network, leading to a parent attachment under a transaction that will never be supported.
This means the best transactions to choose lie somewhere near the frontier, but not too far deep in history.

In adaptive selection, a node starts at the frontier and retreats towards the genesis transaction until it finds an eligible parent.
The frontier transactions are those that currently do not have any children in the node's $\mathcal{T}$.
The set of strongly preferred transactions $\mathcal{E}$ is filtered by an additional criterion that the confidence should be larger than zero. This filters out transactions from unstable conflict set having zero confidence.
If there exist $p$ transactions in the filtered $\mathcal{E}$, then the adaptive selection will just yield them.
%YYY why isn't this bad, for the reasons in the previous paragraph?
Otherwise, the policy tries the parents of the transactions in $\mathcal{E}$, thus increasing the chance of finding more stabilized transactions as it retreats.
The retreating search will terminate when it reaches the genesis transaction.
Formally, the selected parents in this adaptive selection policy is precisely:

\begin{center}
\begin{algorithmic}[1]
    \small
    \Function{parentSelection}{$\mathcal{T}$}
        \State $\mathcal{E}' \coloneqq \{T: d(T) > 0, \forall T\in\mathcal{E}\}$.
        \State \Return $\{T: T \in \mathcal{E}' \land \forall T'\in\mathcal{T}, T \gets T', T' \notin \mathcal{E}'\}$.
    \EndFunction
    \captionof{figure}{Adaptive parent selection.}\label{fig:gossipchain-parent}
\end{algorithmic}
\end{center}
%YYY what are you memoizing and why does this help? Also, can't an attacker create a gazillion nodes at the frontier and dilute your efforts?
The formal definition involves checking the modified frontier condition each
time it retreats and reaches a vertex. In fact, each ``forall'' quantifier
demands an $O(|\mathcal{T}|)$ time, so the overall cost is
$O(|\mathcal{T}|^2)$. However, by doing search from the frontier with
memoization, the quadratic cost could be avoided. Moreover, using an
approximation technique in Section~\ref{sec:pruning}, it is possible to replace the
$|\mathcal{T}|$ by a constant number of transactions in practice.

Attackers cannot suddenly create a surge of vertices at the frontier to dilute
the progress of Snowball, because with the above policy, only the transactions
with positive confidence will be considered as parents. The polling happens via
gossiping, and each query has to wait for the response from $k$ randomly chosen
peers. The pace is then coordinated by all correct nodes. So even if an
attacker increases the fan-out of the DAG, those new vertices will not
get much attention unless its has confidence larger than zero, in which the
progress is not diluted.

